General Incremental Learning with Domain-aware Categorical Representations

Continual learning is an important problem for achieving human-level intelligence in real-world applications as an agent must continuously accumulate knowledge in response to streaming data/tasks. In this work, we consider a general and yet under-explored incremental learning problem in which both the class distribution and class-specific domain distribution change over time. In addition to the typical challenges in class incremental learning, this setting also faces the intra-class stability-plasticity dilemma and intra-class domain imbalance problems. To address above issues, we develop a novel domain-aware continual learning method based on the EM framework. Specifically, we introduce a flexible class representation based on the von Mises-Fisher mixture model to capture the intra-class structure, using an expansion-and-reduction strategy to dynamically increase the number of components according to the class complexity. Moreover, we design a bi-level balanced memory to cope with data imbalances within and across classes, which combines with a distillation loss to achieve better inter- and intra-class stability-plasticity trade-off. We conduct exhaustive experiments on three benchmarks: iDigits, iDomainNet and iCIFAR-20. The results show that our approach consistently outperforms previous methods by a significant margin, demonstrating its superiority.

==> data/discussion.tex <==
\section{Discussion}
\paragraph{Negative Social Impact}
Our method enables model to continuously adapt to novel class- and domain-distribution, which can be leveraged by malicious applications to upgrade its model with incoming data.
Moreover, the continuous adaptation requires extra training cost for the incoming data.

\paragraph{Limitations}
Our method is designed for allowing access to limited old examples, and thus can not be applied to the setting with no memory.
% Training cost?
% assume test distribution is uniform, without estimation of test distribution?

